Memory Makes the Difference: Evaluating How Different Memory Roles Shape Conversational Agents

Prior research on memory mechanism in RAG-based conversational system has emphasized how memory is stored and retrieved. However, far less is known about how memories with different functional roles influence response quality. Specifically, how they shape an agent's responses under varying conversational contexts and whether they lead to substantively different response behaviors. Existing evaluations in conversational system are also largely reference-based, insufficiently capturing the nuances in responses that may address users' preferences differently. In this work, we probe the impact of different memory types in shaping agents' responses. We present a fine-grained taxonomy of conversational memory, classify retrieved memories into different role types, and design a user-centric evaluation framework that simulates user perspectives. Through comparative experiments on long-term datasets and frontier LLMs, our analysis reveal many differentiated effects of memories: e.g., clarifying memory improves responses' factual accuracy and constraint awareness, making them more correct and personalized; irrelevant memory reduces topic relevance and degrades constraint awareness. Despite the power of frontier LLMs, these findings shed light on how different memory types can be leveraged to produce more personalized responses and inspire further research in this direction.

==> tables/improvement_rate_parametric_gpt.tex <==
\begin{table*}
    \centering
    \small
    \renewcommand{\arraystretch}{1.6}
    \setlength{\tabcolsep}{4pt}
    \resizebox{\textwidth}{!}{
    \begin{tabular}{>{\centering\arraybackslash}m{2.6cm}|>{\centering\arraybackslash}m{1.7cm}>{\centering\arraybackslash}m{1.3cm}>{\centering\arraybackslash}m{1.7cm}>{\centering\arraybackslash}m{1.7cm}>{\centering\arraybackslash}m{1.6cm}>{\centering\arraybackslash}m{1.6cm}>{\centering\arraybackslash}m{1.6cm}>{\centering\arraybackslash}m{1.55cm}>{\centering\arraybackslash}m{1.55cm}}
    \Xhline{0.8pt}
    % \rowcolor{gray!30}
    \makecell{\textbf{Comparative}\\\textbf{Experiment} (\vs \parametric)} & \textbf{\makecell{World\\Knowledge}} & \textbf{\makecell{Answer\\Accuracy}} & \textbf{\makecell{Internal\\Coherence}} & \textbf{\makecell{Topic\\Relevance}} & \textbf{\makecell{Constraint\\Awareness}} & \textbf{Completeness} & \textbf{Actionability} & \textbf{\makecell{Memory\\Coverage}}
 & \textbf{\makecell{ROUGE-1\\Recall}} \\ 
    \Xhline{0.8pt}
    \clarifying & $\hlred{0.00}$\vrule $\hlred{0.00}$ & ~~~$\hlwhite{--}$~~ \vrule $\hlgreen{0.96}$ & $\hlred{0.00}$\vrule $\hlwhite{0.50}$ & $\hlwhite{0.56}$\vrule $\hlgreen{1.00}$ & ~~~$\hlwhite{--}$~~\vrule $\hlgreen{1.00}$ & $\hlgreen{0.77}$\vrule $\hlgreen{0.89}$ & $\hlwhite{0.43}$\vrule $\hlwhite{0.53}$ & $\hlgreen{1.00}$\vrule $\hlgreen{0.87}$ & $\hlgreen{1.00}$\vrule $\hlgreen{0.85}$ \\ \hline
    \answer + \clarifying & $\hlred{0.00}$\vrule ~~ $\hlwhite{--}$~~~ & $\hlgreen{0.89}$\vrule $\hlgreen{1.00}$ & $\hlwhite{0.50}$\vrule ~~$\hlwhite{--}$~~~~ & $\hlgreen{0.90}$\vrule $\hlgreen{1.00}$ & $\hlgreen{1.00}$\vrule $\hlgreen{1.00}$ & $\hlgreen{0.93}$\vrule $\hlgreen{0.83}$ & $\hlgreen{0.80}$\vrule $\hlgreen{1.00}$ & $\hlgreen{1.00}$\vrule $\hlgreen{1.00}$ & $\hlgreen{0.92}$\vrule $\hlgreen{1.00}$ \\ \hline
    \enriching & $\hlred{0.26}$\vrule $\hlred{0.04}$ & $\hlgreen{0.80}$\vrule $\hlgreen{0.91}$ & $\hlred{0.00}$\vrule $\hlred{0.14}$ & $\hlgreen{0.82}$\vrule $\hlgreen{0.96}$ & $\hlgreen{0.76}$\vrule $\hlgreen{0.88}$ & $\hlgreen{0.74}$\vrule $\hlgreen{0.75}$ & $\hlred{0.32}$\vrule $\hlgreen{0.69}$ & $\hlgreen{0.85}$\vrule $\hlgreen{0.83}$ & $\hlgreen{0.82}$\vrule $\hlgreen{0.74}$ \\ \hline
    \distracting & $\hlred{0.20}$\vrule $\hlred{0.08}$ & $\hlgreen{0.86}$\vrule $\hlgreen{0.75}$ & ~~~$\hlwhite{--}$~~\vrule $\hlred{0.00}$ & $\hlgreen{0.80}$\vrule $\hlgreen{0.87}$ & $\hlgreen{0.80}$\vrule $\hlgreen{0.77}$ & $\hlgreen{0.70}$\vrule $\hlgreen{0.67}$ & $\hlred{0.27}$\vrule $\hlgreen{0.62}$ & $\hlgreen{0.92}$\vrule $\hlgreen{0.87}$ & $\hlgreen{0.79}$\vrule $\hlgreen{0.60}$ \\ \hline
    \irrelevant & $\hlred{0.26}$\vrule $\hlred{0.09}$ & $\hlwhite{0.50}$\vrule $\hlwhite{0.51}$ & $\hlred{0.00}$\vrule $\hlred{0.29}$ & $\hlgreen{0.68}$\vrule $\hlgreen{0.64}$ & $\hlwhite{0.43}$\vrule $\hlgreen{0.64}$ & $\hlwhite{0.49}$\vrule $\hlwhite{0.46}$ & $\hlred{0.29}$\vrule $\hlred{0.34}$ & $\hlgreen{0.86}$\vrule $\hlgreen{0.72}$ & $\hlgreen{0.75}$\vrule $\hlwhite{0.57}$ \\ \hline
    \answer + \clarifying + \enriching + \distracting + \irrelevant & $\hlred{0.29}$\vrule $\hlred{0.18}$ & $\hlgreen{0.96}$\vrule $\hlgreen{0.97}$ & $\hlred{0.00}$\vrule $\hlred{0.40}$ & $\hlgreen{0.95}$\vrule $\hlgreen{0.96}$ & $\hlgreen{0.97}$\vrule $\hlgreen{0.97}$ & $\hlgreen{0.95}$\vrule $\hlgreen{0.92}$ & $\hlred{0.28}$\vrule $\hlgreen{0.75}$ & $\hlgreen{0.97}$\vrule $\hlgreen{0.88}$ & $\hlgreen{0.93}$\vrule $\hlgreen{0.91}$ \\ \hline
 \Xhline{0.8pt}
    \end{tabular}
    }
    \caption{improvement rate parametric gpt}
    \label{tab:improvement_rate_parametric_gpt}
\end{table*}
